Towards representation agnostic probabilistic programming

Current probabilistic programming languages and tools tightly couple model representations with specific inference algorithms, preventing experimentation with novel representations or mixed discrete-continuous models. We introduce a factor abstraction with five fundamental operations that serve as a universal interface for manipulating factors regardless of their underlying representation. This enables representation-agnostic probabilistic programming where users can freely mix different representations (e.g. discrete tables, Gaussians distributions, sample-based approaches) within a single unified framework, allowing practical inference in complex hybrid models that current toolkits cannot adequately express.

==> ccbm-dbn.tex <==
%\documentclass[tikz]{standalone}
%\usetikzlibrary{arrows}
%\usetikzlibrary{arrows.meta}
%
%\begin{document}
\begin{tikzpicture}[>={Triangle[width=4]},
every edge/.style={->,draw,thick},
trans/.style={blue,thick},
latent/.style={draw,thick,shape=circle,inner sep=0pt,minimum size=30pt},
observed/.style={draw,thick,shape=circle,inner sep=0pt,minimum size=30pt, fill=green!50}, % 
hyper/.style={draw,fill,shape=circle,inner sep=1pt}]
\clip (-1.1,-3.8) rectangle +(8.1,6.8) ;
\fill[fill=black!10,rounded corners=2pt]
    (-0.9,-3.8) rectangle +(3.7,6.8)
    (3.1,-3.8) rectangle +(3.7,6.8)
    ;
\draw[rounded corners=10pt]
    (-0.75,-1.75) rectangle +(3.4,4.45)
    (3.25,-1.75) rectangle +(3.4,4.45)
   ;
\draw
	(-4,0) node {}
    +(0,1) node (at-2) {}
    +(0,-1) node (ft-2) {}
    +(2,2) node (st-2) {}
    +(2,0) node (et-2) {}
%
	(0,0) node {}
    +(-0.75,2.4) node[right] {$X_{t-1}$}
    +(0,1) node[latent] (at-1) {$A_{t-1}$}
    +(0,-1) node[latent] (ft-1) {$\C F_{t-1}$}
    +(0,-3) node[observed] (dt-1) {$\C D_{t-1}$}
    +(2,0) node[latent] (et-1) {$E_{t-1}$}
    +(2,2) node[latent] (st-1) {$S_{t-1}$}
    +(2,-3) node[observed] (yt-1) {$\C Y_{t-1}$}
%
	(4,0) node {}
    +(-0.75,2.4) node[right] {$X_{t}$}
    +(0,1) node[latent] (at) {$A_{t}$}
    +(0,-1) node[latent] (ft) {$ \C F_{t}$}
    +(0,-3) node[observed] (dt) {$ \C D_{t}$}
    +(2,0) node[latent] (et) {$E_{t}$}
    +(2,2) node[latent] (st) {$S_{t}$}
    +(2,-3) node[observed] (yt) {$ \C Y_{t}$}
%
	(8,0) node {}
    +(0,1) node (at1) {}
    +(1,-1) node (ft1) {}
    +(2,2) node (st1) {}
    +(2,-3) node (yt1) {}
%
	(at-2) edge[lightgray,bend right=25] (ft-1)
    (et-2) edge[lightgray] (at-1)
    (et-2) edge[lightgray] (ft-1)
    (at-2) edge[lightgray] (at-1)
    (ft-2) edge[lightgray] (ft-1)
    (st-2) edge[lightgray] (at-1)
    (st-2) edge[lightgray] (st-1)
    (st-2) edge[lightgray,bend left=10] (yt-1)
%
	(at) edge[lightgray,bend right=27] (ft1)
    (at) edge[lightgray] (at1)
    (et) edge[lightgray] (at1)
    (et) edge[lightgray] (ft1)
    (ft) edge[lightgray] (ft1)
    (st) edge[lightgray] (at1)
    (st) edge[lightgray] (st1)
    (st) edge[lightgray,bend left=10] (yt1)
%
    (at-1) edge (et-1)
    (at-1) edge (ft-1)
    (at-1) edge (st-1)
    (at-1) edge[bend left=10] (yt-1)
    (dt-1) edge (ft-1)
    (et-1) edge (st-1)
    (ft-1) edge (et-1)
    (ft-1) edge (yt-1)
    (st-1) edge[bend left=25] (yt-1)
%
	(at-1) edge[trans,bend right=25] (ft)
    (at-1) edge[trans] (at)
    (et-1) edge[trans] (at)
    (et-1) edge[trans] (ft)
    (ft-1) edge[trans] (ft)
    (st-1) edge[trans] (at)
    (st-1) edge[trans] (st)
    (st-1) edge[trans, bend left=10] (yt)
    
    (at) edge (et)
    (at) edge (ft)
    (at) edge (st)
    (at) edge[bend left=10] (yt)
    (dt) edge (ft)
    (et) edge (st)
    (ft) edge (et)
    (ft) edge (yt)
    (st) edge[bend left=25] (yt)
 	;

\end{tikzpicture}
% \end{document}
